ExtremeC3Net: Extreme Lightweight Portrait Segmentation Networks using Advanced C3-modules

Designing a lightweight and robust portrait segmentation algorithm is an important task for a wide range of face applications. However, the problem has been considered as a subset of the object segmentation problem. bviously, portrait segmentation has its unique requirements. First, because the portrait segmentation is performed in the middle of a whole process of many realworld applications, it requires extremely lightweight models. Second, there has not been any public datasets in this domain that contain a sufficient number of images with unbiased statistics. To solve the problems, we introduce a new extremely lightweight portrait segmentation model consisting of a two-branched architecture based on the concentrated-comprehensive convolutions block. Our method reduces the number of parameters from 2.1M to 37.7K (around 98.2% reduction), while maintaining the accuracy within a 1% margin from the state-of-the-art portrait segmentation method. In our qualitative and quantitative analysis on the EG1800 dataset, we show that our method outperforms various existing lightweight segmentation models. Second, we propose a simple method to create additional portrait segmentation data which can improve accuracy on the EG1800 dataset. Also, we analyze the bias in public datasets by additionally annotating race, gender, and age on our own. The augmented dataset, the additional annotations and code are available in https://github.com/HYOJINPARK/ExtPortraitSeg .

==> Eng/Analysis.tex <==
\section{Analysis on EG1800 Dataset}
\label{sec:anlz}
EG1800 dataset \yj{consists of} various 1800 portrait images \yj{collected} from Flickr and \yj{manually generated segmentation labels}.
The dataset covers many different images, but \yj{the analysis below shows that the dataset is biased to the specific races or ages.}
\yj{From Table~\ref{tab:att_num}, we can see that Caucasian occupies majority portion in the dataset. Also, the age group is largely biased to `Youth and Moddle-ages' group.}
We additionally annotated about detail attributes of faces and give a guideline which attribute is more critical to segmentation accuracy from our analysis.


\subsection{Bias in Attributes}
\label{sec:bias}


\begin{table}[t]
  \begin{center}
    \begin{tabular}{| c | l | ccc | }
    \hline
          &       & train & val   & total \\
           \hline \hline
    \multirow{3}[0]{*}{Races} & Caucasian & 1086  & 214   & 1300 \\
          & Asian & 168   & 46    & 214 \\
          & Black & 58    & 11    & 69 \\
           \hline
    \multirow{2}[0]{*}{Gender} & Man   & 516   & 112   & 628 \\
          & Woman & 796   & 159   & 955 \\
           \hline
    \multirow{3}[0]{*}{Ages} & Infant or Child & 130   & 42    & 172 \\
          & Youths or Middle-ages & 1089  & 219   & 1308 \\
          & Seniors & 93    & 10    & 103 \\
           \hline
    \end{tabular}%
    \end{center}
     \caption{Detail classs of attributes about EG1800 dataset}
  \label{tab:att_num}%
\end{table}%



\begin{figure*}[t]
\begin{center}
\includegraphics[width=0.99\linewidth]{Fig/histogram.png}
\end{center}
   \caption{Dataset histogram about the number of each class images.}
\label{fig:att_histo}
\end{figure*}


\begin{table*}[h]
\begin{center}

    \begin{tabular}{| c | ccc | c |ccc | c | ccc |}
    \hline
    Class & Races & Genders & Ages  & Class & Races & Genders & Ages  & Class & Races & Genders & Ages \\
     \hline  \hline
    0     & Caucasian & Man   & Child    & 6     & Asian & Man   & Child     & 12    & Black & Man   & Child  \\
    1     & Caucasian & Man   & Youth   & 7     & Asian & Man   & Youth   & 13    & Black & Man   & Youth \\
    2     & Caucasian & Man   & Senior & 8     & Asian & Man   & Senior & 14    & Black & Man   & Senior \\
    3     & Caucasian & Woman & Child    & 9     & Asian & Woman & Child     & 15    & Black & Woman & Child  \\
    4     & Caucasian & Woman & Youth    & 10    & Asian & Woman &Youth    & 16    & Black & Woman & Youth \\
    5     & Caucasian & Woman & Senior & 11    & Asian & Woman & Senior & 17    & Black & Woman &Senior  \\
      \hline
    \end{tabular}%
      \end{center}
     \caption{Class of attributes. Class of "Child" includes infants or children and class of "Youth" means youths and middle-ages people }
   
  \label{tab:att_label}%
\end{table*}%


The public dataset EG1800\cite{shen2016automatic} 
%is constructed
\Lars{contains} 1800 images dataset for portrait stylizing from segmentation results. 
%However, several links for images are missed, and the available the number of image for train and validation is total 1579.
\Lars{However, many urls are broken and the total amount of available images is 1579.}
We analyzed the attribute of the dataset based on races, gender, ages, and if an image has more than one person, we counted every people.
We annotated the detail classes of the image by six human annotators and the Table\ref{tab:att_num} show the result of our annotation.
We divided dataset 18 classes following to our additional annotation as shown in Table\ref{tab:att_label} and draw histogram to describe bias of this dataset in Figure \ref{tab:att_label}.
Both train and validation set have a severe bias to Caucasian and youth \& middle-aged people, and we could not find any image has a senior black woman.
The more detail result is in supplemental materials.

\subsection{Accuracy depending on attributes}
\label{sec:att}
In this section, we conducted a comparative experiment to comprehend how data augmentation methods could solve data biased problems.
Experiment 1 and 2 have the same structure and use only EG1800 dataset for a train. 
However, they were trained with different data augmentation method.
While, we used naive data augmentation methods such as random resizing, random crop, and random horizontal flip for experiment 1, we applied a more sophisticated data augmentation method proposed by PortraitNet\cite{zhang2019portraitnet}.
The method consists of deformation and texture augmentation methods:

The deformation augmentation method \newline
\textbullet \quad Random horizontal flip \newline
\textbullet \quad Random rotation  $\{-45 ^{\circ} \sim 45 ^{\circ} \}$  \newline
\textbullet \quad Random resizing  $\{0.5 \sim 1.5 \}$  \newline
\textbullet \quad Random translation  $\{-0.25 \sim 0.25 \}$ 

The texture augmentation method \newline
\textbullet \quad Random noise  $\{ \text{Gaussian noise, } \sigma= 10 \}$  \newline
\textbullet \quad Image blur  $\{ \text{kernel size } = 3 \text{ or } 5 \text{ randomly} \}$ \newline
\textbullet \quad Random color change  $\{0.4 \sim 1.7 \}$  \newline
\textbullet \quad Random brightness change  $\{0.4 \sim 1.7 \}$ \newline
\textbullet \quad Random contrast change  $\{0.6 \sim 1.5 \}$ \newline
\textbullet \quad Random sharpness change  $\{0.8 \sim 1.3 \}$ 


\begin{table}[t]
  \begin{center}
    \begin{tabular}{|c|l| ccc |}
    \hline
          &       & Num of img & Exp1 & Exp2 \\
          \hline \hline
    \multirow{3}[0]{*}{race} & Caucasian & 213   & 93.67  & 94.51  \\
          & Asian & 46    & 94.31  & 94.78  \\
          & Black & 11    & 94.74  & 95.05  \\
          \hline
    \multirow{2}[0]{*}{gender} & Man   & 111   & 92.85  & 94.21  \\
          & Weman & 158   & 94.54  & 94.81  \\
          \hline
    \multirow{3}[0]{*}{ages} & Child & 42    & 94.47  & 93.87  \\
          & Youth & 218   & 93.87  & 94.79  \\
          & Senior & 10    & 90.07  & 92.97  \\
          \hline
    \end{tabular}%
    \end{center}
  \label{tab:att_acc}%
  \caption{ Experiment result of different data augmentation method about each attribute from validation set.}
\end{table}%

Surprisingly, there is no significant difference from the bias of races in both experiment 1 and 2.
Both experiment 1 and 2 have similar accuracy for the entire class in races attributes.
However, gender and ages attribute has imbalanced accuracy according to the number of images.
The number of woman images is 280 larger than man images in the train set as shown in Table \ref{tab:att_num} and it induces to make overfitting model about woman's portrait.
The number of child and seniors images lower than youth, but the accuracy of a child is higher than other else, and the accuracy about seniors is remarkably lower than other else.
Therefore, we conjecture that the difference between races is not that important, but genders and ages occur overfitting model depending on a train set in portrait segmentation.
Besides, the property between child and youth is not critical than the senior's property. 

The sophisticated data augmentation method helps to improve the accuracy of the small number of the attribute, but it could not solve every problem.
Low accuracy of man class is got over by data augmentation method, and the accuracy imbalance is reduced in experiment 2, as shown in Table \ref{tab:att_acc}.
However, the bias problem about age attribute is not solved.
The accuracy of seniors is still lower than other class in experiment 2.
We conjecture that the prominent features of the seniors, such as wrinkles and ages spots, are difficult to make by the data augmentation method, as shown in Figure \ref{fig:att_ex}.
Also, the face shape for children and youths is close to the elliptical shape, but the shape of the face deviates from the ellipse as people get older like senior woman's face in Figure \ref{fig:att_ex}.
Therefore, this problem can not be solved, and it is essential about constructing a balanced dataset regarding ages attribute.


% The human's face has different features according to races, ages, genders. 
% Even though we use general data augmentation methods such as scale, illumination, translation, and noise, it is hard to mention we get a new human face feature.
% The original public dataset barely has around 1300 for training, and it cannot reflect all the feature of human's face, and there is severe bias to specific race and ages.
% We analyzed the category of the public dataset and how much effect to segmentation accuracy from the biased dataset.

\begin{figure}[t]
\begin{center}
\includegraphics[width=0.99\linewidth]{Fig/portrait.png}
\end{center}
   \caption{ Example of images of various ages. Row1 : seniors, Row 2: child, youths and middle-ages from left to right }
\label{fig:att_ex}
\end{figure}

